GraphScale: A Framework to Enable Machine Learning over Billion-node Graphs

Graph Neural Networks (GNNs) have emerged as powerful tools for supervised machine learning over graph-structured data, while sampling-based node representation learning is widely utilized in unsupervised learning. However, scalability remains a major challenge in both supervised and unsupervised learning for large graphs (e.g., those with over 1 billion nodes). The scalability bottleneck largely stems from the mini-batch sampling phase in GNNs and the random walk sampling phase in unsupervised methods. These processes often require storing features or embeddings in memory. In the context of distributed training, they require frequent, inefficient random access to data stored across different workers. Such repeated inter-worker communication for each mini-batch leads to high communication overhead and computational inefficiency. We propose GraphScale, a unified framework for both supervised and unsupervised learning to store and process large graph data distributedly. The key insight in our design is the separation of workers who store data and those who perform the training. This separation allows us to decouple computing and storage in graph training, thus effectively building a pipeline where data fetching and data computation can overlap asynchronously. Our experiments show that GraphScale outperforms state-of-the-art methods for distributed training of both GNNs and node embeddings. We evaluate GraphScale both on public and proprietary graph datasets and observe a reduction of at least 40% in end-to-end training times compared to popular distributed frameworks, without any loss in performance. While most existing methods don't support billion-node graphs for training node embeddings, GraphScale is currently deployed in production at TikTok enabling efficient learning over such large graphs.

==> abstract_emb.tex <==
% \begin{abstract}
% Graph Neural Networks (GNNs) have emerged as a powerful tool for supervised machine learning over graph-structured data.
% However, scalability remains a major challenge for training GNNs over large graphs (e.g., >1 billion nodes) with high-dimensional node (and/or edge) features. The scalability bottleneck is due to the mini-batch sampling phase which requires either storing more than a billion features in memory or non-contiguous access to the features if they are stored externally.
% Similarly, unsupervised machine learning methods over large graphs, such as training node embeddings, are unscalable for the same reasons (now, the bottleneck is handling, say, node embeddings, instead of node features). Due to their complicated structure, distributed training over graphs is inefficient and slow due to high communication overheads and heavily relies on the partitioning schemes used to divide the graph data structure. 

% We propose Right-On-Spot (ROS), a framework to store and process large graph data distributedly. The key insight in our design of ROS is the separation of actors (aka workers) who store the data and those who perform the training. This separation allows us to decouple computing and storage in graph training, thus effectively building a pipeline where data fetching and data computation can overlap asynchronously. 
% % Further, due to its serverless storage feature, ROS can scale training effortlessly to billion-node scale graphs by utilizing a larger pool of actors. 
% Our experiments show that ROS outperforms state-of-the-art methods for distributed training of both GNNs and node embeddings. We evaluate ROS both on publicly available graph data as well as industry-scale graph datasets from production systems at TikTok and observe a reduction of at least $40\%$ in end-to-end training times, without any loss in performance. For training node embeddings, most existing methods don't support billion node graphs, but ROS makes it feasible and efficient.
% \end{abstract}

\begin{abstract}
Unsupervised learning methods, such as training node and/or edge embeddings, have emerged as a powerful tool for machine learning on data structured as graphs.
However, scalability remains a major challenge for training such embeddings over large graphs (e.g., >1 billion nodes). 
This is because the scale of such graphs requires distributed training, but the size of the embeddings (aka the machine learning model) prohibits storing and training embeddings in a data-parallel fashion, and traditional model parallel methods are slow due to high communication overheads. 
% Due to their complicated structure, distributed training over graphs is inefficient and slow due to high communication overheads and heavily relies on the partitioning schemes used to divide the graph data structure. 

We propose GraphScale, an algorithm to train node embeddings on billion-node graphs. GraphScale runs a serverless framework to store and process large graph data distributedly. The key insight in our design of ROS is the separation of actors (aka workers) who store the data and those who perform the training. This separation allows us to decouple computing and storage in graph training, thus effectively building a pipeline where data fetching and data computation can overlap asynchronously.
Further, due to its serverless storage feature, ROS can scale training effortlessly to billion-node scale graphs by utilizing a larger pool of actors. 
Our experiments show that ROS outperforms state-of-the-art methods for distributed training embeddings. We evaluate ROS both on publicly available graph data as well as industry-scale graph datasets from production systems at TikTok. For large graphs, most existing methods are not feasible due to their requirement to communicate gradients of the large embeddings matrix. GraphScale makes training such embeddings feasible and efficient. For smaller graphs, we observe a reduction of at least $40\%$ in end-to-end training times with GraphScale, without any loss in performance. 
% For training node embeddings, most existing methods don't support billion node graphs, but ROS makes it feasible and efficient.
\end{abstract}

==> node_emb_training.tex <==
\section{GraphScale for Training Node Embeddings}
\label{sec:ros_emb_design}

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{figures/fig_model_codes.pdf}
\caption{Comparison of Python codes for PyTorch DDP versus GraphScale-based model definitions using PyTorch.}
\label{fig:model_codes}
\end{figure*}

 \begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{figures/fig_training_codes.pdf}
\caption{Comparison of Python codes for DDP versus GraphScale-based graph node embedding training for PyTorch.}
\label{fig:training_codes}
\end{figure*}

% Many unsupervised learning applications require training embedding vectors for nodes which can be computationally expensive or infeasible on a single machine. This is because holding the model in the worker's memory is difficult, especially for present-day graphs where the number of nodes easily scales into the billions.
This section describes the implementation of graph learning algorithms for training graph node embeddings using GraphScale. More specifically, we describe how we utilize GraphScale storage to hold the model distributedly in workers' memory and perform efficient training of large-graph node embeddings.

Two notable node embedding algorithms are: 1) DeepWalk \cite{deepwalk}, which trains node embeddings by generating random walks from each node in the graph and applying the skip-gram model from NLP for context-based training, and 2) LINE \cite{line}, where the objective function utilizes information from both the local and global graph structures around a node  to learn its embedding. We use these algorithms to illustrate training with GraphScale. \yy{Do we have to boil down to two specific embedding methods, Deepwalk and Line? Can you make it sound more general by going with skip-gram-based node embedding methods, such as deepwalk and line?}

{\bf Notation}: Say we have a graph $\G = (V, E)$ with $N= |V|$ nodes and $|E|$ edges, and the embedding dimension for each node is $d$. The objective is to learn the node embeddings matrix $\M \in \R^{|V|\times d}$. Matrix $\M$ may be large enough that it may not fit into the memory of a worker. Further, during training a mini-batch with $B$ source nodes, let $n$ be the maximum number of nodes obtained during graph sampling (including source nodes in mini-batch and their positively and negatively sampled nodes). 
The number $n$ is typically easy to estimate, e.g., for DeepWalk, it is $B \times $ {\tt walk\_len}, where {\tt walk\_len} is the length of the random walk used for DeepWalk training, and for LINE, it is $B \times (2 + {\tt num\_neg})$, where {\tt num\_neg} is the number of negatively sampled nodes per source node in the mini-batch.
We typically have $N \gg n$, that is, the total number of nodes in the graph is much greater than the number of nodes sampled in a mini-batch.

PyTorch's DistributedDataParallel (DDP) is a commonly used method of training machine learning models distributedly in a data-parallel fashion. We use DDP training as a baseline to explain the process of training node embeddings using GraphScale. In figures \ref{fig:model_codes} and \ref{fig:training_codes}, we describe the python codes for the model definition and training loops, respectively, for both DDP and GraphScale-based training. Our implementations are on top of PyTorch, and the differences in the implementations for both methods are highlighted in yellow. 

 \yy{I don't quite get the takeaway of this comparison. Yes, GraphScale and DDP are implemented differently, and they differ in those highlighted lines. But how do these differences show the superiority of GraphScale? Or how do these differences imply? } \vg{Maybe I an highlight this properly, but the point of it was to show that GraphScale is easy to implement with a few lines of changes to code.}
Fig. \ref{fig:model_codes} shows the common aspects of model definitions shared by DDP and GraphScale. In line 4, the PyTorch embeddings are initialized (however, with different sizes). In lines 5 and 6 in the GraphScale case, we initialize the GraphScale storage for node embeddings and momentum vector, respectively, where the dimension of GraphScale matrices is $N \times d$. This initializes the embeddings and momentum matrices distributedly using Ray. In line 11, {\tt compute\_loss} is a generic loss function that computes the loss using the current batch (which includes the source and positively and negatively sampled nodes). For example, in the case of DeepWalk, the batch contains random walks over source nodes, and the training loss over each walk is computed using the SkipGram model as described in the original paper \cite{deepwalk}. 
% Popular models such as DeepWalk and LINE are already implemented as a part of the continuously evolving GraphScale python library.

Fig. \ref{fig:training_codes} describes the pseudo-code for DDP and GraphScale-based PyTorch training loop. Note that the implementation for GraphScale-based training is as straightforward as only a few lines of code changes. The most notable points are:
\begin{itemize}[leftmargin=*]
\setlength{\parskip}{0pt}
\setlength{\itemsep}{0pt}
    \item The size of the embedding matrix in {\tt ddp\_model} is $N \times d$ (Line 1, Fig. \ref{fig:training_codes}). When $N = 2$ billion and $d=128$, the size of the embedding matrix is 1 TB when stored in 32-bit precision. This can easily exceed the capacity of the most powerful machines. In comparison, the {\tt ros\_model} has an embedding matrix of dimension $n \times d$, where $N \gg n$, e.g., $n = 5000$ when the mini-batch size, $B = 1000$, and the walk length is 5 in DeepWalk.
    \item The {\tt ddp\_model} is wrapped around the {\tt DistributedDataParallel} class of PyTorch to enable data-parallel training (Line 2, Fig. \ref{fig:training_codes}). This implies that gradients are averaged before the model update in each iteration. Thus, in our experiments in Sec. \ref{sec:ros_exps}, we observe DDP training incurs huge communication costs when compared to GraphScale-based training, which translates to a lower training efficiency. 
    \item Minimal changes in the training loop are required when migrating from DDP to GraphScale-based training (Fig. \ref{fig:training_codes}). 
    \item In the case of GraphScale, the loss is computed using the embeddings of nodes that are a part of the local subgraph for that mini-batch (that is, the nodes obtained after sampling) and not the entire graph (Line 11, Fig. \ref{fig:model_codes}).
    \item GraphScale cannot use PyTorch's optimizer out-of-the-box since the model and momentum updates require updating the values in GraphScale storage. Hence, we have a custom optimizer  for GraphScale (Line 8, Fig. \ref{fig:training_codes} and Fig. \ref{fig:ros_momentum_update}). We have implemented popular optimizers such as SGD with momentum \cite{sgd_momentum} and Adam \cite{adam} as a part of the GraphScale package.
\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/fig_ros_momentum_update.pdf}
\caption{Python code for SGD with momentum update when both the embeddings and momentum vectors are stored in GraphScale storage.}
\label{fig:ros_momentum_update}
\end{figure}

In Fig. \ref{fig:ros_momentum_update}, we describe our implementation of model update in GraphScale for SGD with momentum. In Line 3, we obtain the gradient of the embedding vectors for nodes that are a part of the subgraph. In Line 7, we multiply the momentum data in GraphScale by the momentum value using the GraphScale {\tt mult()} operation. In Line 11, we add the gradient corresponding to the nodes in the batch to update the momentum vector for that iteration using the GraphScale {\tt put()} operation. Finally, in Line 18, the Ray actors perform an SGD update of the model by first multiplying the momentum data by the learning rate and then subtracting it from the current model data using the {\tt mult\_add()} operation. Note that {\tt mult()} and {\tt mult\_add()} operations are completed by multiple Ray storage actors parallelly that store data (e.g., model and momentum) in their local memory and, thus, do not require any raw data communication. Finally, functions such as {\tt get()}, {\tt put()}, {\tt mult()} and {\tt mult\_add()} are implemented in the GraphScale library for performing basic operations over GraphScale data (see Fig. \ref{fig:ros_operations} for details). 

\begin{figure}[t]
\centering
\includegraphics[width=0.38\textwidth]{figures/ros_operations.pdf}
\caption{An illustration of a few basic operations implemented in the GraphScale library, where each Ray actor stores a shard of the embedding and momentum data in two separate GraphScale data structures. Trainer can use {\tt get()} ({\tt put()}) to receive (write) data to GraphScale. Operations {\tt mult()},  and {\tt mult\_add()} are performed locally in actors' memory and in a parallel fashion.}
\label{fig:ros_operations}
\end{figure}

\textbf{Synchronization}. There are two types of synchronizations required: across iterations and across trainers. 
To achieve synchronization across iterations, we add a barrier after the write operation at the end of each iteration (that is, after the trainers update embedding and momentum). This barrier allows trainers to read updated values for the next iteration. 
During the write operation, synchronization is also required among parallel trainers (as they might be updating embeddings for the same nodes). However, we do not apply strict synchronization between the trainers because we observe that the incurred error is reasonably tolerable. We evaluate the convergence of training with GraphScale in Section \ref{sec:ros_exps_emb} and show that it performs on par with data-parallel training.

% \begin{table}
% \begin{center}
% \begin{tabular}{ |p{2.5cm}||p{5cm}|  }
% %{0.5\textwidth} { | >{\centering\arraybackslash}X || >{\centering\arraybackslash}X |  }
% %\hline
% %\multicolumn{2}{|c|}{GraphScale's APIs} \\
%  \hline
%  APIs & Description \\
% \hline
% \hline
%  {\tt get(Vids)}  & It returns the values from the given vertex IDs.  \\
% \hline
%  {\tt \small{put(Vids,Vals)}}  & It updates the data using the given vertex IDs and values. \\
% \hline
%  {\tt mult(Vids, a)}  & It multiplies the values of the associated vertex IDs with the parameter a and the update the values.  \\
% \hline
% {\tt mult\_add(Vids, a, b)}  & After applying the mult operation, it add another parameter b to update the values.  \\
% \hline
% \end{tabular}
% \caption{GraphScale's API}
% \label{table:ros_api}
% \end{center}
% \end{table}




% \begin{table*}
% \begin{center}
% \begin{tabular}{ |p{0.8cm}|p{2.4cm}|p{2.6cm}|p{2.6cm}|p{2.6cm}|p{2.6cm}|  }
%  \hline
%   & Attributes & GraphLearn (GL) & PyTorch DDP & PyTorch BigGraph & GraphScale \\
%  \hline\hline
%  \multirow{4}{4em}{Read} & Decouple of metadata and raw data & No, they are tightly coupled. & No, it does not distingush them. & No, it does not distingush them.  & Yes, they are completely separated. \\
%  \cline{2-6}
%  & Avoid frequent data movement & No, data has to go through proxy. & No, data movement is frequent among processes. & No, it is based on client/server mode. & Yes, directly from server to trainer. \\
%   \cline{2-6}
%  & Request batching and aggregation & No, each request may incur cross node communication. & No, no relevant interface is provided. & No, it does not support this. & Yes, it always batch request and aggregate vertex IDs. \\
%   \cline{2-6}
%  & Async operation for prefetch & Yes, prefetch is enabled by default \cite{bytegnn}. & No, no relevant interface is provided. & No, it does not support this. & Yes, trainer can initiate data transfer anytime. \\
% \hline

% \multirow{3}{4em}{Write} & Support of partial model update & Read-only & No, lack of support of model parallelism & Yes \xc{???} & Yes, easy APIs are provided. \\
%  \cline{2-6}
% & Avoid back-forth operation per update & Read-only & Yes, because it uses allreduce for update. & No, it needs a read followed by an update. & No, but both are efficient. \\
%  \cline{2-6}
% & Low communication cost & Read-only & No, due to the cost of data parallelism & Maybe \xc{???} & Yes, due to our design. \\
% \hline
% \end{tabular}
% \caption{Comparison among GL, PyTorch DDP, PyTorch BigGraph and GraphScale. }
% \label{table:ros_comparison}
% \end{center}
% \end{table*}

%{\bf Comparison with Existing Frameworks}.
%Table \ref{table:ros_comparison} summarizes all differences between GraphScale and existing frameworks on two types of operations: read and write. When training GNN algorithms, we rely the high efficiency of read operation for feature fetching. When training node embedding algorithms, we need to use both read and write operations.\rh{I feel the last sentence is out of place.}


\textbf{Implementation}. We implement GraphScale on top of Ray \cite{ray} using the actor model.
The implementation takes 2.8K lines of code (LoC) using Python and 0.5K LoC with C++. GraphScale leverages Ray's flexible scheduling capability so that users can easily use asynchronous operations and pipelines.
The C++ implementation is to optimize the indexing and construction of large data arrays.
% Table.\ref{table:ros_api} lists current APIs exposed for training. The remaining sections presents how to train graph embedding with these APIs.

==> paper_emb.tex <==
\section{Introduction}
\label{intro}

Graph learning is a powerful way to generalize traditional deep learning methods onto graph-structured data that contains interactions (that is, edges) between individual units (that is, nodes). Despite the promising performance of machine learning methods that learn directly from graph data \cite{gnn_review_book, gcn}, their adaption at modern web companies has been limited due to the sheer scale \cite{pbg_biggraph}. 
For example, the social network graph at Facebook includes over two billion
user nodes and over a trillion edges \cite{fb_graph_scale}, the users-products graph at Alibaba consists of more than a billion users and two billion items \cite{wang_alibaba}, and the user-to-item graph at Pinterest includes at least 2 billion entities and over 17 billion edges \cite{pinterest_embedding}. At Bytedance, we frequently observe graphs with over a billion nodes on data obtained from the social media platform TikTok.
%\xc{Risk control at Bytedance/TikTok has a graph of 1 billion nodes and 92 billion edges that needs for graph learning.}
This paper proposes Righ-On-Spot (ROS) as a framework to tackle the scale of modern-day graphs for efficient machine learning over graph-structured data.

% Machine learning on graphs can be broadly classified into two categories. The {\bf first} is supervised learning, where the training process ingests the node features, edge features, graph structure, etc., and the labels for the supervised learning task at hand, for example, node classification, link prediction, and graph clustering. Graph Neural Networks (GNNs) have become the de-facto way of supervised learning on graphs, popularized by methods such as Graph Convolution Network (GCN) \cite{gcn} and GraphSAGE \cite{graphsage}. GNNs have been applied to a broad range of applications, such as recommendation systems \cite{recommender_gcn} and drug discovery \cite{drug_discovery}, to obtain state-of-the-art results.

% One critical bottleneck for mini-batch training of GNNs is the sampling phase, where for each vertex in the mini-batch, the sampler samples and fetches a subset of its neighbors and their corresponding features. The sampling phase can take a significantly longer time than the training phase due to a large amount of random data access and remote feature fetching, especially during distributed training of large graphs \cite{bytegnn, gns_da, mlsys_gnn_sampling, liu2021bgl}. 

%In ROS, we separate the feature-fetching and node-sampling phases, so that we can do aggregated communications within each phase. This optimization contributes to substantial improvements in both throughput and latency.



% \vg{Add a figure like Figure 1 in Sancus (VLDB best paper), where we show that distributed fetching of features can result in a lot of cross-device communication. Paper: https://www.vldb.org/pvldb/vol15/p1937-peng.pdf}

% The {\bf second} broad category is unsupervised learning to train graph embedding vectors.
Working with graph data directly, especially for the purposes of machine learning, is complex, and thus, a common technique is to use graph embedding methods to create vector representations for each node.
Node embedding methods are a way to convert graph data into a more computationally tractable form to allow them as an input to a variety of machine learning tasks \cite{hamilton2017representation}.
The representations can then serve as useful features for downstream tasks such as recommender systems \cite{wang_alibaba}, link prediction \cite{deepwalk}, predicting drug interactions \cite{bio_zitnik}, community detection \cite{community_detection}, etc. Hence, such methods are getting significant traction in both academia and industry \cite{embedding_framework}.

One limitation of training node embeddings for graphs using traditional methods is that it requires storing embedding vectors in memory. Such methods typically use data-parallelism (as illustrated in Fig. \ref{fig:graph_dp}), 
where the graph is partitioned across nodes using partitioning schemes, e.g., Metis \cite{metis}, and the entire model (in this case, the node embedding matrix) is held in memory. For example, an embedding model for a graph with one billion nodes and an embedding dimension of 128 would require 512 GB of memory to store just the parameters in 32-bit precision floats. Further storing the momentum vector would require storage space of a similar order. This renders training node embedding for large graphs infeasible for large graphs on most servers due to storage constraints\footnote{Note that learning the node embeddings happens only for transductive methods. The embedding vectors are not trained for inductive methods, such as unsupervised Graphsage \cite{graphsage}. Instead, a neural network is trained to output embedding vectors for graph nodes based on their neighborhood subgraph.}. 
% or unreasonably slow if external storage is used for the purposes of storing intermediate embedding vectors during training

When storing the embedding matrix in memory is feasible, data-parallel training is further limited due to an allreduce operation to average the gradients after every iteration (as illustrated in Fig. \ref{fig:graph_dp}), 
which results in substantial communication costs (see experiments in Sec. \ref{sec:ros_exps_emb}). To ameliorate this, model-parallelism methods have been proposed in the literature that further partition the large model across multiple workers \cite{zero}. However, compared to data-parallelism, model-parallel methods typically take at least twice the time to train due to increased communication costs \cite{deepspeed, dct_kdd}. On the other hand, ROS utilizes the property that only a small subset of nodes are updated in each iteration to outperform both data-parallel and model-parallel training. 


\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/graphs_data_parallel.pdf}
\caption{\footnotesize Data parallel training of node embedding matrix where each trainer stores one graph partition. It is required that each worker has enough memory to hold the entire embedding matrix. Further, high communication cost is incurred during allreduce while averaging gradients in each iteration.}
\label{fig:graph_dp}
\end{figure}


This paper proposes a serverless framework called Right-On-Spot (ROS) to address and mitigate key bottlenecks for applying machine learning over large graphs. 
The key idea of ROS is to separate data storage and tensor computation to speed-up machine learning over large-scale graph data. The key features of ROS are:
\begin{itemize}[leftmargin=*]
\setlength{\parskip}{0pt}
\setlength{\itemsep}{0pt plus 0.2pt}

    % \item {\bf Fast feature-fetching}: GNN training algorithms involve two inputs: the graph topology and the features associated with vertices and edges. In terms of byte sizes, the features are significantly larger than topology. For example, in for the ogbn-Papers100M dataset \cite{ogb}, the feature vector size is $4\times$ the size of graph topology. Therefore feature fetching tend to become the bottleneck in most cases.
    
    % To address this, ROS disassociates the feature fetching from sampling by separating the computation and storage. The features are stored distributedly in the memory of workers, and thus, the amount of storage space available scales with the number of workers.
    \item {\bf Training large-graph node embeddings feasible}: For data-parallel training, each worker has to store the entire node embeddings in memory. To address the bottleneck of limited storage while training node embeddings for large graphs, ROS stores embeddings (and other auxiliary data such as the momentum and variance for the optimizers such as Adam \cite{adam}) in distributed memory of workers, which allows the training of node embeddings  to scale linearly with the number of workers.  It further reduces the communication required to aggregate gradients in each iteration by order of magnitude.
    \item {\bf Serverless}: ROS is a serverless library built on top of Ray \cite{ray}. Being serverless, it has features such as elasticity in terms of the number of workers and failure tolerance. Thus, the resources can be provisioned in real-time when doing training over a large graph and taken care of through a simple API provided by Ray.
    \item {\bf Simplicity}: We have designed ROS such that integrating it with the existing graph training code is very convenient and typically done using a few lines of code. Also, ROS is graph backend agnostic and can work with multiple graph frameworks such as DGL, PyTorch-geometric, and graphlearn. Furthermore, it does not rely on any partitioning algorithm.
\end{itemize}

% One of our key contributions is to extend the Graph learning system design by using a serverless paradigm. Dorylus \cite{dorylus} is a related previous work that uses AWS Lambda to build a part serverless GNN training system. Our work is the first one that adapts and fully utilizes an existing state-of-the-art serverless framework rather than building everything from scratch. Note there is a strong trend of using new hardware such as GPUs and TPUs for graph learning. We believe the new hardware will soon be better supported by generic serverless frameworks. When it happens, our design can be easily extended to an even wider spectrum of system design options and keep evolving on top of that. Thus, the trend of new hardware is orthogonal to our contributions through ROS. Finally, we train node embeddings on an industry dataset where training with existing methods is infeasible due to the scale. 

The rest of the paper is organized as follows. In Sec. \ref{sec:ros_design}, we review the basics of GNN training, motivate ROS's design, and conclude by describing ROS's system architecture. In Sec. \ref{sec:ros_emb_design}, we extend ROS to  training node embedding for large-scale graphs in a parallel fashion.
In Sec. \ref{sec:ros_exps}, 
we compare ROS with several state-of-the-art graph learning methods in our experiments. In Sec. \ref{sec:ros_exps_gnn}, we show that training GNNs with ROS is at least $30\%$ faster than state-of-the-art GNN training systems like DistDGL \cite{dist_dgl} and Graphlearn (also known as AliGraph) \cite{aligraph}. In Sec. \ref{sec:ros_exps_emb}, we compare ROS for training node-embeddings in large graphs against existing methods and observe up to $73\%$ savings.
% data-parallel training and PyTorch-BigGraph (PBG) \cite{pbg_biggraph}. 
% PBG is a recently proposed node embedding training system that aims to mitigate the memory bottleneck while training over large graphs. 
 % when training node embeddings on large graphs with ROS. 
Finally, we use ROS to train node embeddings on an industry-scale dataset where training with existing methods is not feasible due to the scale. 

% \begin{figure}
% \centering
% \includegraphics[scale=0.22]{result_figures/overview_comp.jpg}
% \label{fig::overview_comp}
% \caption{Three major phases of GNN training are shown at the top. At the bottom-left are the three key physical components for GNN training. For instance, GL and DistDGL includes {\tt A} and {\tt C}. PyTorch BigGraph includes {\tt B} and {\tt C}. ROS (at bottom-right) is designed to cover all three components.}
% \end{figure}

\section{ROS: An Overview}
\label{sec:ros_design}
In this section, we first review the basics of GNN training. Then, we motivate the design goals of ROS, followed by describing its system architecture.
% We review feature fetching step and training step with Graph learn, PyTorch BigGraph and PyTorch DDP. 

\subsection{Motivations and Goals}
% Mini-batch processing in Graph Neural Network (GNN) training can be divided into three main steps: (1) Sampling a subgraph from the original graph. The result is the vertex and edge IDs of the sampled nodes and edges, respectively. (2) Feature fetching corresponding to vertex/edge IDs of the sampled nodes/edges in the sub-graph, and (3) Training the GNN for that mini-batch using the sub-graph topology, and the features and labels for corresponding nodes and edges.


% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.24]{no_watermark/Flowchart.jpg}
% %\includegraphics[scale=0.2]{result_figures/GL_arch.jpg}
% \caption{Graph service is a component for sampling and feature fetching in GL. Each trainer is designated to a proxy node that handles data collection. %A generic K/V store shares the same architecture for the storage of graph data, which is the case of DistDGL.
% }
% \label{fig:gl_feature_fetch}
% \end{figure}
% \setlength{\textfloatsep}{8.0pt}

% {\bf I/O bottleneck from feature fetching}. 
% Existing GNN training frameworks suffer from data I/O bottlenecks. Two representative distributed GNN training frameworks  Graphlearn (GL) \cite{aligraph} and DistDGL \cite{dist_dgl}. A further optimization to GL is ByteGNN \cite{bytegnn}, where sampling and feature fetching can be parallelized, and the k-hops can be pipelined. DistDGL is based on a generic K/V store to fetch features. Internally, the two frameworks share the same architecture (as illustrated in Fig. \ref{fig:gl_feature_fetch}).

% These designs all share a similar procedure of feature fetching. For each request per mini-batch, the respective backend issues a request to fetch features for the sampled vertices. The request is routed to the related proxy, which then fetches the features according to the sharding strategy. The proxy collects the data, then sent back to the trainer.  

% This design is inefficient due to two reasons. First, it requires a large number of requests to fetch data for a single batch, which might cause significant network congestion. Second, the two requests of two neighboring hops are highly likely to have duplicate vertices due to the power-law attribute of the graph. Each vertex may be included in multiple requests leading to a heavy network workload. 
% %We give a specific example of this at the end of next section.

% Let us take the GraphSage \cite{graphsage} model training as an example to compare the difference between GL and ROS. A fanout of [15, 10] means there are 2 hops of vertices to retrieve: 15 neighbors for the first hop, and 10 neighbors for the second hop, respectively. For each hop, there are three types of sampler: seed sampler, positive sampler, and negative sampler. In Fig. \ref{fig:gl_feature_fetch}, there are 5 links, where 4 links are from server to proxy and 1 from proxy to trainer. 
% Therefore, we have to issue at least $3\times3\times5=45$ requests to fulfill a single batch task. Thus, GNN training using existing backends is bottlenecked by the data I/O phase  \cite{bytegnn, mlsys_gnn_sampling, gns_da}.
% As we explained in the next section (and illustrated in Fig. \ref{fig:ros_design_fig}), ROS only needs one request for K-hops and all samplers. It bypasses the proxy for data movement with only 4 links. In total, only 4 requests are needed for a batch. 
% Further, combined with request batching and aggregation, ROS can significantly reduce I/O workload.




{\bf Design goals of ROS}:
%The bottleneck of IO mentioned above, motivates us to develop a system to enable training with more efficient I/O. 
ROS is designed to tackle the I/O bottleneck problem we discussed above. We want to achieve the following goals:
%ROS is designed to tackle the I/O bottleneck problem we discussed above fundamentally. The following summarizes three perspectives resulting in the problem, which also serve as our design goal.

\begin{itemize}[leftmargin=*]
\setlength{\parskip}{0pt}
\setlength{\itemsep}{0pt}
    \item Efficient random access: The nature of the graph learning algorithm leads to lots of random data access (e.g., while feature-fetching during the sampling phase). 
    % Randomness is mandatory for the i.i.d. of the sampled subgraph. 
    In a distributed setup, cross-machine communication is also inevitable due to the multi-hop pattern of the graph, which is also random. 
    \item High throughput: Mini-batch training  GNN models may require a larger number of features for each read/write operation (especially to support larger batch sizes). Hence, we want higher throughput.
    \item High concurrency of data access: We would like to support multiple trainers reading and writing simultaneously. 
    % \item Simple APIs to customize graph learning logic: This requires the support of update operations such as adding and multiplying to the stored data. Further, these APIs should be easily integrable into existing code. 
\end{itemize}
In our design of ROS, we address all the challenges above. 
%Next, we present the system architecture of ROS in detail.



\subsection{ROS: System Architecture}

\begin{figure}[h]
\centering
%\includegraphics[scale=0.2]{result_figures/ROS_design.jpg}
\includegraphics[scale=0.23]{no_watermark/Flowchart-2.jpg}
\caption{ROS overview. MetaActor is responsible for data sharding, and ObjectActor stores the raw data. Trainers are the clients that read/write data in parallel. The thin line is the metadata flow, the dashed line represents the synchronization among MetaActor, and the solid line is the raw data flow.}
\label{fig:ros_design_fig}
\end{figure}

Fig. \ref{fig:ros_design_fig} illustrates the system design of ROS. 
% Our insight to these challenges above is to design a generic and unified framework for all the data we may need during the GNN training, including features, embeddings and momentum. 
It supports data partitioning efficient data retrieval and data update. ROS's design principles include the three points below.


{\bf 1. Separate metadata and raw data}:
Metadata can be vertex indices, the ObjectActor ID, the shard index, or a reference to the raw data. The raw data can be any data type we support here, such as vertex features and embeddings.
As shown in Fig. \ref{fig:ros_design_fig}, two types of data flows correspond to the two types. 
The MetaActor stores the mapping between the vertex IDs to the IDs of ObjectActor. The ObjectActor stores the  raw data in memory. \\
{\bf 2. Minimize data movement}:
We believe that any raw data movement between MetaActor and ObjectActor is unnecessary. 
MetaActor is only responsible for retrieving the mappings. 
ObjectActor handles the data movement directly to trainers. 
If there is any update to the raw data, ObjectActor processes the update locally. \\
{\bf 3. Batching requests and data aggregation}:
Request batching and data aggregation are designed to save network bandwidth further. 
On the trainer side, we aggregate vertices to deduplicate vertex IDs before sending a request to MetaActor.
On the ObjectActor side, we construct a single data block per request and give it to the trainer, letting it initiate the data-flow illustrated by the data flow in Fig. \ref{fig:ros_design_fig}.




Next, we describe how the ROS system architecture supports basic operations such as reading and writing.
During the {\bf read operation}, 
The trainer first buffers all requests per training batch and deduplicates the vertices before sending the request to MetaActor. Each trainer is designated to a MetaActor for load balancing. It will route all requested vertex IDs to the corresponding ObjectActor. Once the requests are received, the ObjectActor constructs a data block and returns a reference to the trainer. The trainer then starts the data transfer from all ObjectActors asynchronously.

%reduce the number of internal requests and avoid unnecessary data movement.
During the {\bf update operation}, 
the trainer first retrieves the mapping information from MetaActor. The new values will be partitioned based on the mapping and then written to ObjectActor. Here, each ObjectActor maintains a sorted list of keys to speed up the lookup process. 
Since we have multiple MetaActors, the new mapping will be automatically synchronized among them. This process happens asynchronously while the data is being written to the ObjectActors; thus, it incurs almost no overhead.

ROS also supports some other simple computations, such as add and multiply. These operations are similar to the update operation we described above. 
The only difference is that once the ObjectActor receives the new data, the simple computations happen locally and then update the values. The next section describes these operations in detail, where we utilize ROS for node embedding training.


\section{ROS for Training Node Embeddings}
\label{sec:ros_emb_design}
Many unsupervised learning applications require training embedding vectors for nodes which can be computationally expensive or infeasible on a single machine. This is because holding the model\footnote{Note that in this section, we use the term ``model'' interchangeably with graph node embeddings.} in the worker's memory is difficult, especially for present-day graphs where the number of nodes easily scales into the billions. This section describes the implementation of graph learning algorithms for training graph node embeddings using the ROS functionality. More specifically, we describe how we utilize the ROS storage feature to hold the model distributedly in workers' memory and make training of large-graph node embeddings feasible.

Two notable node embedding algorithms are: 1) DeepWalk \cite{deepwalk}, which trains node embeddings by generating random walks from each node in the graph and applying the skip-gram model from NLP for context-based training, and 2) LINE \cite{line}, where the objective function utilizes information from both the local and global graph structures around a node  to learn its embedding. We use these algorithms to illustrate training with ROS and further present results for these two popular node embedding methods in our experiments in Sec. \ref{sec:ros_exps_emb}.

% When the number of nodes is large (think billions), training graph node embeddings using traditional data-parallel training is infeasible since it is difficult to hold the model in the worker's memory. Next, we will describe in detail how we utilize the ROS storage feature to hold the model distributedly in workers' memory and make training of large-graph node embeddings feasible.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{figures/fig_model_codes.pdf}
\caption{Comparison of Python codes for PyTorch DDP versus ROS-based model definitions using PyTorch.}
\label{fig:model_codes}
\end{figure*}

{\bf Notation}: Say we have a graph $\G = (V, E)$ with $N= |V|$ nodes and $|E|$ edges, and the embedding dimension for each node is $d$. The objective is to learn the node embeddings matrix $\M \in \R^{|V|\times d}$. Matrix $\M$ may be large enough that it may not fit into the memory of a worker. Further, during training a mini-batch with $B$ source nodes, let $n$ be the maximum number of nodes obtained during graph sampling (including source nodes in mini-batch and their positively and negatively sampled nodes). 
The number $n$ is typically easy to estimate, e.g., for DeepWalk, it is $B \times $ {\tt walk\_len}, where {\tt walk\_len} is the length of the random walk used for DeepWalk training, and for LINE, it is $B \times (2 + {\tt num\_neg})$, where {\tt num\_neg} is the number of negatively sampled nodes per source node in the mini-batch.
We typically have $N \gg n$, that is, the total number of nodes in the graph is much greater than the number of nodes sampled in a mini-batch.

PyTorch's DistributedDataParallel (DDP) is a commonly used method of training machine learning models distributedly in a data-parallel fashion. We use DDP training as a baseline to explain the process of training node embeddings using ROS. In figures \ref{fig:model_codes} and \ref{fig:training_codes}, we describe the python codes for the model definition and training loops, respectively, for both DDP and ROS-based training. Our implementations are on top of PyTorch, and the differences in the implementations for both methods are highlighted in yellow. 

Fig. \ref{fig:model_codes} shows the common aspects of model definitions shared by DDP and ROS. In line 4, the PyTorch embeddings are initialized (however, with different sizes). In lines 5 and 6 in the ROS case, we initialize the ROS storage for node embeddings and momentum vector, respectively, where the dimension of ROS matrices is $N \times d$. This initializes the embeddings and momentum matrices distributedly using Ray. In line 11, {\tt compute\_loss} is a generic loss function that computes the loss using the current batch (which includes the source and positively and negatively sampled nodes). For example, in the case of DeepWalk, the batch contains random walks over source nodes, and the training loss over each walk is computed using the SkipGram model as described in the original paper \cite{deepwalk}. Popular models such as DeepWalk and LINE are already implemented as a part of the continuously evolving ROS python library.

 \begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{figures/fig_training_codes.pdf}
\caption{Comparison of Python codes for DDP versus ROS-based graph node embedding training for PyTorch.}
\label{fig:training_codes}
\end{figure*}

Fig. \ref{fig:training_codes} describes the pseudo-code for DDP and ROS-based PyTorch training loop. Note that the implementation for ROS-based training is as straightforward as only a few lines of code changes. The most notable points are:
\begin{itemize}[leftmargin=*]
\setlength{\parskip}{0pt}
\setlength{\itemsep}{0pt}
    \item The size of the embedding matrix in {\tt ddp\_model} is $N \times d$ (Line 1, Fig. \ref{fig:training_codes}). When $N = 2$ billion and $d=128$, the size of the embedding matrix is 1 TB when stored in 32-bit precision. This can easily exceed the capacity of the most powerful machines. In comparison, the {\tt ros\_model} has an embedding matrix of dimension $n \times d$, where $N \gg n$, e.g., $n = 5000$ when the mini-batch size, $B = 1000$, and the walk length is 5 in DeepWalk.
    \item The {\tt ddp\_model} is wrapped around the {\tt DistributedDataParallel} class of PyTorch to enable data-parallel training (Line 2, Fig. \ref{fig:training_codes}). This implies that gradients are averaged before the model update in each iteration. Thus, in our experiments in Sec. \ref{sec:ros_exps}, we observe DDP training incurs huge communication costs when compared to ROS-based training, which translates to a lower training efficiency. 
    \item Minimal changes in the training loop are required when migrating from DDP to ROS-based training (Fig. \ref{fig:training_codes}). 
    \item In the case of ROS, the loss is computed using the embeddings of nodes that are a part of the local subgraph for that mini-batch (that is, the nodes obtained after sampling) and not the entire graph (Line 11, Fig. \ref{fig:model_codes}).
    \item ROS cannot use PyTorch's optimizer out-of-the-box since the model and momentum updates require updating the values in ROS storage. Hence, we have a custom optimizer  for ROS (Line 8, Fig. \ref{fig:training_codes} and Fig. \ref{fig:ros_momentum_update}). We have implemented popular optimizers such as SGD with momentum \cite{sgd_momentum} and Adam \cite{adam} as a part of the ROS package.
\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/fig_ros_momentum_update.pdf}
\caption{Python code for SGD with momentum update when both the embeddings and momentum vectors are stored in ROS storage.}
\label{fig:ros_momentum_update}
\end{figure}

In Fig. \ref{fig:ros_momentum_update}, we describe our implementation of model update in ROS for SGD with momentum. In Line 3, we obtain the gradient of the embedding vectors for nodes that are a part of the subgraph. In Line 7, we multiply the momentum data in ROS by the momentum value using the ROS {\tt mult()} operation. In Line 11, we add the gradient corresponding to the nodes in the batch to update the momentum vector for that iteration using the ROS {\tt put()} operation. Finally, in Line 18, the Ray actors perform an SGD update of the model by first multiplying the momentum data by the learning rate and then subtracting it from the current model data using the {\tt mult\_add()} operation. Note that {\tt mult()} and {\tt mult\_add()} operations are completed by multiple Ray ObjectActors parallelly that store ROS data like model and momentum in their local memory and do not require any raw data communication. Finally, functions such as {\tt get()}, {\tt put()}, {\tt mult()} and {\tt mult\_add()} are implemented in the ROS library for performing basic operations over ROS data (see Fig. \ref{fig:ros_operations} for details). 

\begin{figure}[t]
\centering
\includegraphics[width=0.38\textwidth]{figures/ros_operations.pdf}
\caption{An illustration of a few basic operations implemented in the ROS library, where each Ray actor stores a shard of the embedding and momentum data in two separate ROS data structures. Trainer can use {\tt get()} ({\tt put()}) to receive (write) data to ROS. Operations {\tt mult()},  and {\tt mult\_add()} are performed locally in ObjectActors' memory and in a parallel fashion.}
\label{fig:ros_operations}
\end{figure}

\textbf{Synchronization}. There are two types of synchronizations required: across iterations and across trainers. 
To achieve synchronization across iterations, we add a barrier after the write operation at the end of each iteration (that is, after the trainers update embedding and momentum). This barrier allows trainers to read updated values for the next iteration. 
During the write operation, synchronization is also required among parallel trainers (as they might be updating embeddings for the same nodes). However, we do not apply strict synchronization between the trainers because we observe that the incurred error is reasonably tolerable. We evaluate the convergence of training with ROS in Section \ref{sec:ros_exps_emb} and show that it performs on par with data-parallel training.

% \begin{table}
% \begin{center}
% \begin{tabular}{ |p{2.5cm}||p{5cm}|  }
% %{0.5\textwidth} { | >{\centering\arraybackslash}X || >{\centering\arraybackslash}X |  }
% %\hline
% %\multicolumn{2}{|c|}{ROS's APIs} \\
%  \hline
%  APIs & Description \\
% \hline
% \hline
%  {\tt get(Vids)}  & It returns the values from the given vertex IDs.  \\
% \hline
%  {\tt \small{put(Vids,Vals)}}  & It updates the data using the given vertex IDs and values. \\
% \hline
%  {\tt mult(Vids, a)}  & It multiplies the values of the associated vertex IDs with the parameter a and the update the values.  \\
% \hline
% {\tt mult\_add(Vids, a, b)}  & After applying the mult operation, it add another parameter b to update the values.  \\
% \hline
% \end{tabular}
% \caption{ROS's API}
% \label{table:ros_api}
% \end{center}
% \end{table}




% \begin{table*}
% \begin{center}
% \begin{tabular}{ |p{0.8cm}|p{2.4cm}|p{2.6cm}|p{2.6cm}|p{2.6cm}|p{2.6cm}|  }
%  \hline
%   & Attributes & GraphLearn (GL) & PyTorch DDP & PyTorch BigGraph & ROS \\
%  \hline\hline
%  \multirow{4}{4em}{Read} & Decouple of metadata and raw data & No, they are tightly coupled. & No, it does not distingush them. & No, it does not distingush them.  & Yes, they are completely separated. \\
%  \cline{2-6}
%  & Avoid frequent data movement & No, data has to go through proxy. & No, data movement is frequent among processes. & No, it is based on client/server mode. & Yes, directly from server to trainer. \\
%   \cline{2-6}
%  & Request batching and aggregation & No, each request may incur cross node communication. & No, no relevant interface is provided. & No, it does not support this. & Yes, it always batch request and aggregate vertex IDs. \\
%   \cline{2-6}
%  & Async operation for prefetch & Yes, prefetch is enabled by default \cite{bytegnn}. & No, no relevant interface is provided. & No, it does not support this. & Yes, trainer can initiate data transfer anytime. \\
% \hline

% \multirow{3}{4em}{Write} & Support of partial model update & Read-only & No, lack of support of model parallelism & Yes \xc{???} & Yes, easy APIs are provided. \\
%  \cline{2-6}
% & Avoid back-forth operation per update & Read-only & Yes, because it uses allreduce for update. & No, it needs a read followed by an update. & No, but both are efficient. \\
%  \cline{2-6}
% & Low communication cost & Read-only & No, due to the cost of data parallelism & Maybe \xc{???} & Yes, due to our design. \\
% \hline
% \end{tabular}
% \caption{Comparison among GL, PyTorch DDP, PyTorch BigGraph and ROS. }
% \label{table:ros_comparison}
% \end{center}
% \end{table*}

%{\bf Comparison with Existing Frameworks}.
%Table \ref{table:ros_comparison} summarizes all differences between ROS and existing frameworks on two types of operations: read and write. When training GNN algorithms, we rely the high efficiency of read operation for feature fetching. When training node embedding algorithms, we need to use both read and write operations.\rh{I feel the last sentence is out of place.}


\textbf{Implementation}. We implement ROS on top of Ray \cite{ray} using the actor model.
The implementation takes 2.8K lines of code (LoC) using Python and 0.5K LoC with C++. ROS leverages Ray's flexible scheduling capability so that users can easily use asynchronous operation and pipeline.
The C++ implementation is to optimize the indexing and construction of large data arrays.
% Table.\ref{table:ros_api} lists current APIs exposed for training. The remaining sections presents how to train graph embedding with these APIs.


%\subsection{Fast Training GNNs with ROS and system-level comparison}
%A mini-batch processing while Graph Neural Network (GNN) training can be divided into three main steps: 1) Sampling a subgraph from the original graph. The result is the vertex and edge IDs of the sampled nodes and edges, respectively. 2) Reading features corresponding to vertex/edge IDs of the sampled nodes/edges in the sub-graph, and 3) Training the GNN for that mini-batch using the sub-graph topology, and the features and labels for corresponding nodes and edges. 
%As discussed earlier, feature fetching can quickly become a bottleneck for GNN training due to discontinuous data access. Further, depending on the specific operations, such as multi-hop sampling, a read operation can involve cross-node communication during distributed training. To ameliorate this, we propose ROS storage whose aim is to provide an intermediate layer for efficient reading of features. 

\section{Experimental Results}
\label{sec:ros_exps}

% \begin{table*}
% \begin{center}
% \begin{tabular}{ |m{4cm}|m{4.5cm}|m{5.5cm}| }
%  \hline
%  Configurations & ROS GNN TRaining & ROS Node Embedding Training\\
% \hline
% \hline
%  {\tt Dataset}  & Reddit\cite{redditdata} & ogbn-products, ogbn-papers \cite{ogb},\cite{ogbndata}\\ 
% \hline
%  {\tt Algorithm}  & Unsupervised GraphSage and supervised GraphSage & Deepwalk, LINE\\
% \hline
%  {\tt Baseline}  & Graphlearn (GL), DGL & PyTorch DDP, PyTorch-BigGraph\\
% \hline
%  {\tt Number of machines}  & 4  & 4 \\
% \hline
% {\tt Number of trainers}  & 2 per machine  & 2 per machine \\
% \hline
% {\tt Batch size}  & 512 & 512\\
% \hline
% {\tt Number of epochs } & 4 & 4\\
% \hline
% {\tt Optimizer (Learning rate)} & Adam ($0.003$) & Adam (0.01) for DeepWalk, Adam (1.0) for LINE\\
% \hline
% {\tt Algorithm specific configuration } & The number of hops is 3. Sampling fanout is to specify the number of neighbors per hop. By default, the fanout is (15, 10). & For DeepWalk, the walk-length is 5 and the window-size is 3. LINE uses 5 negative nodes per source node.\\
% \hline
% \end{tabular}
% \caption{Experiments configurations}
% \end{center}
% \end{table*}
To evaluate ROS's performance, we divide our experiments into two parts: GNN algorithms and GE algorithms, respectively, in Section \ref{sec:ros_exps_gnn} and Section \ref{sec:ros_exps_emb}.  On GNN algorithms, we compare ROS against GL and DistDGL. On GE algorithms, we compare ROS with PyTorch DDP and PyTorch BigGraph.


{\bf Experimental setup}: Each machine has 48 physical cores and 700 Gigabytes of memory with Debian 9.13. 
Our distributed setup comprises a cluster of 4 machines connected with 25G/sec ethernet. 
The versions of Ray, PyTorch, and DistDGL are 1.13, 1.12, and 0.9.1, respectively.
The dataset used in our experiments are: Reddit \cite{graphsage}, ogbn-products and ogbn-papers \cite{ogb}.


{\bf Configuration}:
Unless mentioned otherwise, we use the following as the default configurations. The batch size is 512. The number of epochs is 4. The number of trainers per machine is 2.
The optimizer is Adam. The learning rate ($0.003$) for GraphSage, ($0.01$) for DeepWalk, and ($1.0$) for LINE. The sampling fanout is [15, 10]. 


% \subsection{Training GNNs with ROS}
% \label{sec:ros_exps_gnn}
% This section evaluates the performance of ROS on GNN training algorithms, specifically unsupervised and supervised GraphSage.
% All the experiments in this section were performed on the publicly available Reddit graph dataset, which has 232,965 nodes with node feature dimensions of 602. 
% The experiments are conducted to answer the following three questions:
% (1) What is the throughput of feature fetching? (2) How is the latency and the stability? (3) How is the end-to-end performance compared to DistDGL including all three steps sampling, feature fetching and training?


% {\bf Efficient feature fetching}: 
% To precisely evaluate the throughput performance, we only perform sub-graph sampling and feature-fetching but ignore the downstream operations of training. We run unsupervised GraphSage and report the throughput as the number of vertices/keys that it can read per second.  

% We vary two variables to evaluate ROS's scalability: number of trainers and sampling fanout.
% The number of trainer is the parallel number of trainer doing feature fetching.
% The sampling fanout represents the workload per batch. With a batch size of 512 and 3 samplers, there are ${512\times3\times(1 + 1\times15 + 1\times15\times10) = 254k}$ vertices that need to do the feature fetching in each batch.



% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.235\textwidth}
%         \centering
%         \includegraphics[scale=0.36]{result_figures/th_single.pdf}
%         \caption{Single machine.}
%         \label{fig:ff_single}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.235\textwidth}
%         \centering
%         \includegraphics[scale=0.36]{result_figures/th_cluster.pdf}
%         \caption{A cluster of 4 machines.}
%         \label{fig:ff_cluster}
%     \end{subfigure}
% \caption{Throughput (in million vertices per second) during sampling and feature fetching on unsupervised GraphSage with the Reddit dataset. ROS increases the throughput up to $4\times$ when compared to GL.}
% \label{fig:th_single}
% \end{figure} 


% Fig. \ref{fig:ff_single} presents the single machine results.
% With the number of trainers increasing from 1 to 8, ROS has a steady growth while GL has a small throughput increase. With 8 trainers, ROS has a throughput that is $3.73\times$ of GL's.
% Next, we vary the sampling fanout from [10, 5] to [20, 15]. We can clearly see the two trends for GL and ROS. Unlike GL, the throughput increases gradually for ROS. For the fanout of [20, 15], ROS has a throughput of $4\times$ the throughput of GL.

% Fig. \ref{fig:ff_cluster} presents the results on a cluster of four machines.
% When increasing the number of trainers, ROS has a stable growth of throughput from 4 trainers to 16 trainers while GL has a slight growth. Comparing the throughput of 16 trainers with the throughput of 4 trainers, GL increases the throughput by 53\% while ROS increases it by 93\%. With 16 trainers, ROS achieves $3.23\times$ higher throughput. 
% When increasing the sampling fanout, ROS has a solid throughput growth while GL gains not as much. Comparing the fanout [10, 5] with [20, 15], ROS increases the throughput by 69.7\% while GL only increases 4.5\%. On the fanout of [20, 15], ROS has a throughput 3.56 times of GL's. 


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.235\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{result_figures/latency_single.pdf}
%         \caption{Single machine.}
%         \label{fig:latency_single}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.235\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{result_figures/latency_cluster.pdf}
%         \caption{A cluster of 4 machines.}
%         \label{fig:latency_cluster}
%     \end{subfigure}
% \caption{Percentile time of only sampling and feature fetching on the cluster using unsupervised GraphSage with 4 epochs. P99 means the time when $99\%$ of the requests are fulfilled. ROS achieves much better stability than GL; thus, prefetch and pipeline become easier for downstream training.}
% \label{fig:latency}
% \end{figure} 

% {\bf Stable performance}:
% Next, we run unsupervised GraphSage training to show ROS has stable performance for each mini-match. We report the latency of the sampling and the feature fetching per mini-batch. To demonstrate the stability of ROS, we report two percentile statistics: 99 percentile and 80 percentile. 

% Fig. \ref{fig:latency_single} presents the latency on a single node.
% The latency of ROS is more sustainable when the number of trainers increases.
% When comparing P99 percentile times using 8 trainers, ROS is only 2.78\% of GL's time. ROS achieves much higher throughput because ROS avoids data congestion.
% When increasing the sampling fanout, the latency increases almost linearly for all three percentiles for GL, while for ROS it only increases by a tiny portion. For instance, on the fanout [20, 15], ROS's P99 is about 4.1\% of GL's P99 time. 

% Fig. \ref{fig:latency_cluster} shows the latency on the cluster.
% Increasing the number of trainers and the sampling fanout, the latency pattern for both GL and ROS is similar to what we saw on the single machine. GL's two percentile time increases dramatically while ROS's time increases a small portion. On the fanout [20,15], ROS's P99 time is 5.4\% of GL's. 



% {\bf End-to-end performance improvement}:
% When considering end-to-end performance, we feed the features generated from ROS to PyTorch training. Both GL and DistDGL provide the capability of prefetch to pipeline the I/O cost with training computation. We developed a similar pipeline mechanism on top of ROS using Python thread pool.

% We run GraphSage for 4 epochs and report the throughput performance. Regarding the training quality, we validate that the test accuracy on both DistDGL and ROS are the same at 92\%, which is consistent with the results in the original GraphSage paper \cite{graphsage}. 
% We report the throughput with the number of batches per second by varying the number of trainers and the sampling fanout as shown in Fig. \ref{fig:ros_e2e_perf}. 

% When the number of trainers increases, the throughput of both DistDGL and ROS grows proportionally. On average, ROS increases the training throughput by $71.7\%$.
% When the sampling fanout increases, both DistDGL and ROS have reduced throughput because both feature-fetching and training time increase due to the growing workload. On average, ROS improves DistDGL's throughput by 73.8\%.
% %The improvement becomes smaller as the fanout grows. This is because the current implementation uses a Python thread pool. We can achieve a better speedup with a C++ thread pool for pipelining as an optimization.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.235\textwidth}
%         \centering
%         \includegraphics[scale=0.36]{result_figures/e2e_th_trainer.pdf}
%         %\caption{Training throughput.}
%         \label{fig:e2e_perf_trainer}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.235\textwidth}
%         \centering
%         \includegraphics[scale=0.36]{result_figures/e2e_th_fanout.pdf}
%         %\caption{Training throughput.}
%         \label{fig:e2e_perf_fanout}
%     \end{subfigure}
% \caption{End-to-end (including sampling, feature fetching, and training) throughput comparison (number of batches per second) between DistDGL and ROS on supervised Graphsage with the Reddit dataset. ROS doubles Dist DGL's throughput when fanout is (10, 10).}
% \label{fig:ros_e2e_perf}
% \end{figure} 

% %In short, we can see that ROS shows much better scalability than GL regarding both parallelism and data sizes. As we scale up the number of trainers or increase the data sizes, ROS consistently achieves a stable increase of throughput while GL gains a slight increase or even a saturated increase. This is because of ROS design, which schedules the data movement more efficiently and avoids data congestion.

\subsection{Node Embedding Training with ROS}
\label{sec:ros_exps_emb}

In this section, we evaluate the performance of ROS on training node embeddings of graphs through experiments on several real-world datasets. From publicly available datasets, we use a medium-size dataset called ogbn-products and the largest publicly available homogeneous graph dataset called ogbn-papers100M \cite{ogb}. ogbn-products is an undirected graph that has approximately 2.5 million nodes and 62 million edges and represents an Amazon product co-purchasing network, while ogbn-papers100M has 111 million nodes and 1.6 billion edges and is a directed graph representing a paper citation network. Finally, we also implement ROS-based node embedding on an industry-scale dataset with 1 billion nodes and 92 billion edges.  

Throughout the node embedding experiments, we use a Ray cluster of 4 machines. We use two trainers on each machine while training. We perform our experiments on two popular node embedding algorithms, DeepWalk and LINE, to show the efficacy of ROS-based node embedding training. We use a learning rate of 0.01 with Adam optimizer and 1.0 with SGD with momentum for DeepWalk and LINE, respectively, with a batch-size of 512 for both algorithms. We use a walk-length of 5 and a window-size of 3 for DeepWalk; and 5 negative nodes per source node for LINE.

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.5]{figures/iter_ogbn-products_losses_parts4_trainers8_epochs10_size128_lr0.01_bs512.pdf}
        \caption{Training loss for DeepWalk.}
        \label{fig:128_prod_deepwalk_iter}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.23]{figures/time_ogbn-products_losses_parts4_trainers8_epochs10_size128_lr0.01_bs512.pdf}
        \caption{Training time for DeepWalk.}
        \label{fig:128_prod_deepwalk_time}
    \end{subfigure}
        \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.5]{figures/iter_ogbn-products_line_losses_parts4_trainers4_epochs5_size128_lr1_bs512full.pdf}
        \caption{Training loss for LINE.}
        \label{fig:128_prod_line_iter}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.23]{figures/time_ogbn-products_line_losses_parts4_trainers4_epochs5_size128_lr1_bs512full.pdf}
        \caption{Training time for LINE.}
        \label{fig:128_prod_line_time}
    \end{subfigure}
    \caption{Training stats with the ogbn-products graph dataset for an embedding size of 128. ROS has the same accuracy as PyTorch DDP but takes at least $39\%$ less time.}
\label{fig:prod_128}
\end{figure*} 


\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.5]{figures/iter_ogbn-papers_losses_parts4_trainers4_epochs5_size32_lr0.01_bs512.pdf}
        \caption{Training loss for DeepWalk.}
        \label{fig:128_papers_deepwalk_iter}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.23]{figures/time_ogbn-papers_losses_parts4_trainers4_epochs5_size32_lr0.01_bs512.pdf}
        \caption{Training time for DeepWalk.}
        \label{fig:128_papers_deepwalk_time}
    \end{subfigure}
        \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.5]{figures/iter_ogbn-papers_line_losses_parts4_trainers4_epochs5_size32_lr1_bs512.pdf}
        \caption{Training loss for LINE.}
        \label{fig:128_papers_line_iter}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.235\textwidth}
        \centering
        \includegraphics[scale=0.23]{figures/time_ogbn-papers_line_losses_parts4_trainers4_epochs5_size32_lr1_bs512.pdf}
        \caption{Training time for LINE.}
        \label{fig:128_papers_line_time}
    \end{subfigure}
    \caption{Training stats with the ogbn-papers graph dataset for an embedding size of 128. ROS has the same accuracy as PyTorch DDP but takes at least $43\%$ less time.}
\label{fig:papers_128}
\end{figure*} 

{\bf ROS outperforms data-parallel training}: In Fig. \ref{fig:prod_128} and \ref{fig:papers_128}, we plot the training loss for ROS and DDP with respect to (w.r.t.) the number of batches processed and the amount of time taken for the ogbn-products and ogbn-papers100M datasets. For ogbn-products, the embedding size was kept at 128; for ogbn-papers100M, the embedding size was 32. The training statistics were averaged over three independent trials. We highlight two key observations below.\\
1. {\bf Training Loss:} ROS has similar (if not better) training accuracy when compared with DDP. This is evident from figures \ref{fig:128_prod_deepwalk_iter} and \ref{fig:128_prod_line_iter} where we plot the smoothened training loss for DeepWalk and LINE, respectively, on the ogbn-products dataset. The same observation applies for figures \ref{fig:128_papers_deepwalk_iter} and \ref{fig:128_papers_line_iter} where we repeat the experiments for the ogbn-papers100M dataset.\\
2. {\bf Training Runtime}: ROS is significantly faster than DDP. This is evident from figures \ref{fig:128_prod_deepwalk_time} and \ref{fig:128_prod_line_time} for ogbn-products with DeepWalk and LINE algorithms, respectively, and we observe savings of $39\%$ and $68\%$, respectively. Further, from figures \ref{fig:128_papers_deepwalk_time} and \ref{fig:128_papers_line_time} for the ogbn-papers100M dataset, we observe savings of $43\%$ for DeepWalk and $73\%$ for LINE, respectively.

\begin{figure}[!htb]
\includegraphics[scale=0.6]{figures/bar_plot_comp_comm.pdf}
\caption{Runtime comparison for computation and communication phases with ROS and DDP for DeepWalk and LINE on the ogbn-products dataset (with embedding size 128). We observe commensurate savings with computation and communication.}
\label{fig:bar_plot_comp_comm}
\end{figure}

\begin{figure}[!htb]
\includegraphics[scale=0.29]{figures/bar_plot_diff_emb_sizes.pdf}
\caption{Total runtime comparison for different embedding sizes training DeepWalk on the ogbn-products dataset. Savings with ROS increase with embedding size due to less communication and computation when compared to DDP.}
\label{fig:bar_plot_diff_emb_sizes}
\end{figure}

\begin{figure}
\includegraphics[scale=0.6]{figures/bar_plot_pbg.pdf}
\caption{Total runtimes for PBG, DDP and ROS on the ogbn-products and ogbn-papers100M datasets for DeepWalk to achieve the same training loss. PBG is worse than both DDP and ROS due to slower convergence and under-utilization of resources.}
\label{fig:bar_plot_pbg}
\end{figure}

{\bf ROS saves both communication and computation time}: In Fig. \ref{fig:bar_plot_comp_comm}, we compare the average computation and communication time per iteration for ROS with DDP. Computation time primarily comprises of the forward and backward passes, and communication time comprises the optimizer and model updates (that is, allreduce in the case of DDP and ROS storage updates in the case of ROS). We note that ROS outperforms DDP significantly during both communication and computation. During communication, for large embedding sizes, the gradients become large too, and PyTorch DDP requires a lot of communication during allreduce. On the other hand, by virtue of only training nodes in the mini-batch and its sampled neighbors (that is, the subgraph for that mini-batch), ROS reduces the amount of communication required. During computation, ROS further takes less time since it performs operations (such as forward and backward passes) on a PyTorch tensor of the size of the subgraph, while DDP performs these operations on the entire embedding matrix. On a side note, we can also see that DeepWalk spends more time in communication, while LINE requires more time in computation.

{\bf ROS is scalable}: In Fig. \ref{fig:bar_plot_diff_emb_sizes}, we plot the runtimes for the ogbn-products dataset with DDP and ROS for different embedding sizes and observe that ROS performs better as the embeddings get larger. ROS is slower for small embedding sizes since it requires two rounds of communication in each iteration, one for copying the current embedding values from ROS to memory and the second for updating the model in ROS after training. On the other hand, PyTorch DDP requires only one round of communication when the gradients are averaged. However, DDP is not scalable since it requires both higher communication and computation as it operates on the entire DDP matrix (as shown in Fig. \ref{fig:bar_plot_comp_comm} and explained earlier).

{\bf Comparison with PBG}: PyTorch-BigGraph (PBG) was proposed in \cite{pbg_biggraph} to mitigate the issue of memory bottleneck during the training of graph node embeddings by dividing nodes of the graph into buckets equal to the number of machines, say $M$. This divides the edges into $M^2$ buckets depending on the source and destination nodes. Thus, it enables large-scale embedding training when embeddings don't fit in memory by limiting training to disjoint edge buckets. PBG uses a lock server, a parameter server, a partition server, and a shared filesystem to facilitate different aspects of training. This system architecture is complicated and can be cumbersome to implement in production environments. 

In Fig. \ref{fig:bar_plot_pbg}, we observe that to reach the same training loss of 4.45 after starting with the same model values, PBG takes significantly more time than DDP and ROS. This can be attributed to the following reasons. In PBG, the sampling of edges is not i.i.d. since it samples only from the local bucket. Further, the distribution of negatively-sampled edges is different due to local sampling. Finally, since there is a restriction in PBG that requires only one machine to work on one partition of nodes, the training is not embarrassingly parallel, resulting in an under-utilization of resources.

{\bf Training on an industry-scale dataset}: Finally, we train DeepWalk on a proprietary industry-scale dataset at TikTok with approximately 1 billion nodes and 92 billion edges. We use SGD with momentum with a learning rate of 0.01 and a batch-size of 2048. Distributed training is performed on a Ray cluster with 10 machines, where each machine has 700 GB of memory. With an embedding size of 64, the size of the node embedding matrix becomes 256 GB. Storing it along with the graph topology (and the momentum vector) at each node makes PyTorch DDP training infeasible. Thus, we employ ROS, which requires that each node holds one-tenth of the embedding matrix (25.6 GB in this case). 

% ROS can train when embeddings can't fit in memory, while PyTorch DDP can't. Model parallel techniques can be employed with DDP when models are too large to fit in memory, but model parallelism generally increases training time due to extra communication. On the other hand, ROS relies on the unique property of graph training, where only nodes in the subgraph are touched in each iteration; thus, the entire model doesn't need to be stored in memory.

Note that we did not implement any known optimizations to reduce communication during data-parallel training (such as gradient sparsification) or to improve sampling time during GNN training (as discussed in the next section in detail) since they can be applied complementarily to ROS as well, and the focus here was on the key system innovations of ROS. Further, DDP can be made feasible with model parallelism; however, it is known that it increases the time to train by $2\times$ due to additional communication.

\section{Related Work}



% PyTorch BigGraph, Marius, DeepSpeed ZeRO, ByteGNN/Graphlearn (for feature fetching)

%Since dealing with graph data can be quite complicated, dedicated systems have been developed for machine learning on graph data, such as Deep Graph Library (DGL) \cite{dgl}, PyTorch Geometric (PyG) \cite{pyg} and GraphLearn \cite{aligraph}. For GNN training, the algorithm takes two inputs: the graph topology and the features associated with vertices and edges. Typically, the size of the features is significantly larger than the size of the graph topology. For example, in ogbn-Papers100M \cite{ogb}, the feature vector dimension for a vertex is 128, and the size of features is $4\times$ the size of graph topology.

Many single-machine systems have been proposed in the literature to tackle the sampling bottleneck in GNN training. PyTorch-Geometric \cite{pyg} implements a message-passing API for GNN training. Using the Apache TVM compiler, FeatGraph \cite{hu2020featgraph} generates optimized kernels for GNN operators for both CPU and GPU. PaGraph \cite{pagraph} proposes a GPU caching policy to address the subgraph data loading bottleneck. NextDoor \cite{nextdoor} proposes a graph-sampling approach called transit-parallelism for load balancing and caching of edges. \cite{gns_da} propose Global Neighborhood Sampling (GNS) for mixed CPU-GPU training, where a cache of nodes is kept in the GPU through importance sampling, allowing for the in-GPU formation of mini-batches. 
\cite{mlsys_gnn_sampling} uses a performance-engineered neighborhood sampler to mitigate mini-batch preparation and transfer bottlenecks in GPU-based GNN training.
We note that many of the above schemes for faster sampling for GNN training can be used complementarily with ROS.

The above single-machine systems are limited by CPU/GPU memory when processing large industrial-scale graphs.
For GNN training on such large graphs, distributed training was utilized in DistDGL \cite{dist_dgl} and GraphLearn \cite{aligraph}. However, it introduces a key performance bottleneck: high sampling time due to random data access and remote feature fetching. As noted from our experiments in Sec \ref{sec:ros_exps_gnn}, ROS is able to mitigate this bottleneck by separating the topology and feature storage in graphs. 

%Recently, Dorylus \cite{dorylus} proposed a distributed system that uses Amazon EC2 and serverless Lambdas to increase scalability at low cost by pipelining graph and tensor computation-related tasks. 

Even though being a critical problem in the industry, the research for node-embedding training of large graphs is still in its nascent phase. Authors in \cite{nimble_tt_decomp} propose the use of tensor-train decomposition \cite{tt-decomp} to compress embeddings by enabling their compact parametrization. This method can easily be incorporated into node embedding training with ROS to further reduce memory and communication bottlenecks. Marius \cite{marius} was proposed for a single machine GPU training of node embeddings to reduce the data movement by leveraging partition-caching and buffer-aware data orderings.

To the best of our knowledge, the literature around distributed node embedding training for large graphs is limited to PyTorch-BigGraph (PBG) \cite{pbg_biggraph}. PBG proposed a distributed solution but complicated partition-aware distributed training that is not embarrassingly parallel. Also, it requires a large shared parameter server to store the node embeddings while training. Further, they support only a specific loss function rather than all popular methods, such as DeepWalk and LINE. As we observed in our experiments in Sec. \ref{sec:ros_exps_emb}, ROS outperforms PBG due to a better parallelization strategy that utilizes the sub-graph structure while storing the node embeddings distributedly.
% DeepSpeed ZeRO proposes a framework for simultaneous data and model parallel training, but as we illustrate in the paper, it is slower than ROS since it does not take advantage of the problem structure of graph embedding training, where in each iteration, the mini-batch training implies that we update only a part of the model and not the entire model, unlike traditional neural networks. 

\section{Conclusions and Future Work}

We propose ROS, a generic framework for GNN training that can support graph features, node embeddings and momentum in one unified and elegant serverless abstraction. Performance wise, 
the major advantages of ROS are of two-folds: efficient I/O operations and memory footprints. By using GraphSage, Deepwalk and Line algorithms on various datasets, we have demonstrated that ROS has clear advantages over GL, DistDGL and PyTorch BigGraph. 

While ROS is generic and performant, there are various new opportunities to craft better and broader graph learning applications. One direction is to fully utilize GPU training in a serverless system design. 
%This require additional support to move data between RAM and GPU efficiently. 
Another direction is to design an adaptive synchronization policy, so that as a serverless graph learning framework, ROS can support different graph learning algorithms' requirement of model synchronization during training. Additionally, we are planning to use ROS to design an efficient serverless graph model serving system.
% Finally, ROS  Last one is fault tolerance support.

==> ros_overview_detailed.tex <==


\section{GraphScale: An Overview}
\label{sec:ros_design}
In this section, we first review the basics of GNN training. 
% Then, we motivate the design goals of GraphScale, followed by describing its system architecture.
Then, we describe GraphScale and show how it assists in fast distributed GNN training.
% We review feature fetching step and training step with Graph learn, PyTorch BigGraph and PyTorch DDP. 

\subsection{Motivations and Goals}
Mini-batch processing in Graph Neural Network (GNN) training can be divided into three main steps: (1) Sampling a subgraph from the original graph. The result is the vertex and edge IDs of the sampled nodes and edges, respectively. (2) Feature fetching corresponding to vertex/edge IDs of the sampled nodes/edges in the sub-graph, and (3) Training the GNN for that mini-batch using the sub-graph topology, and the features and labels for corresponding nodes and edges.


% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.24]{no_watermark/Flowchart.jpg}
% %\includegraphics[scale=0.2]{result_figures/GL_arch.jpg}
% \caption{Graph service is a component for sampling and feature fetching in GL. Each trainer is designated to a proxy node that handles data collection. For each request per mini-batch, the respective backend issues a request to fetch features for the sampled vertices. The request is routed to the related proxy, which then fetches the features according to the sharding strategy. The proxy collects the data and then sends it back to the trainer.  
% %A generic K/V store shares the same architecture for the storage of graph data, which is the case of DistDGL.
% }
% \label{fig:gl_feature_fetch}
% \end{figure}
% \setlength{\textfloatsep}{8.0pt}

% {\bf I/O bottleneck from feature fetching}. Existing GNN training frameworks suffer from data I/O bottlenecks. 
% % Two representative distributed GNN training frameworks are 
% The two notable distributed GNN training systems, Graphlearn (GL)\footnote{ByteGNN \cite{bytegnn} is a further optimized version of Graphlearn, where sampling and feature fetching are phases of GNN training are parallelized, and the k-hop neighbor fetching is pipelined.} \cite{aligraph} and DistDGL \cite{dist_dgl}, both rely on a similar underlying architecture for feature fetching.
% % (as illustrated in Fig. \ref{fig:gl_feature_fetch}).
% % DistDGL is based on a generic K/V store to fetch features. 
% For each sampling request per mini-batch, the respective graph backend issues a request to fetch features for the sampled vertices.
% % We observe a common limitation in both frameworks. 
% This design is inefficient due to two reasons. First, it processes a large number of requests to fetch features for a single batch, which might cause significant network congestion.
% Second, the requests of neighboring hops are highly likely to have duplicate vertices due to the power-law attribute of the graph, but features for each vertex may be included in multiple requests leading to a heavy network workload. 
% %We give a specific example of this at the end of next section.

{\bf I/O bottleneck during feature fetching}. Current distributed training frameworks for GNNs suffer from data communication bottlenecks. Both Graphlearn (GL) \footnote{ByteGNN \cite{bytegnn} is a further optimized version of Graphlearn, where sampling and feature fetching are phases of GNN training are parallelized, and the k-hop neighbor fetching is pipelined.} \cite{aligraph} and DistDGL \cite{dist_dgl}, which are prominent distributed GNN training systems, exhibit a shared architectural approach in feature fetching. The process involves issuing requests from the graph backend to retrieve features for sampled vertices in each mini-batch. This methodology is inefficient for two primary reasons. Firstly, it generates a high volume of feature-fetching requests for each batch, potentially causing high network traffic. Secondly, due to the graph's power-law distribution, there is a high probability of duplicated vertices in neighboring hops. However, the system often processes features for these repeated vertices multiple times, resulting in increased network load. By the virtue of separating storage and computation, GraphScale significantly reduces the communication overhead by making only one request for features in the sub-graph at each computation actor. 

% Let us take the GraphSage \cite{graphsage} model training as an example to understand the communication bottleneck in distributed GNN training.
% % compare the difference between GL and GraphScale. 
% A fanout of [15, 10] means there are 2 hops of vertices to retrieve: 15 neighbors for the first hop, and 10 neighbors for the second hop, respectively. For each hop, there are three types of samplers: seed sampler, positive sampler, and negative sampler. In Fig. \ref{fig:gl_feature_fetch}, there are 5 links, where 4 links are from server to proxy and 1 from proxy to trainer. 
% Therefore, we have to issue at least $3\times3\times5=45$ requests to fulfill a single batch task. Thus, GNN training using existing backends is bottlenecked by the data I/O phase  \cite{bytegnn, mlsys_gnn_sampling, gns_da}.
% As we explained in the next section (and illustrated in Fig. \ref{fig:ros_design_fig}), 
% GraphScale only needs one request for K-hops and all samplers. It bypasses the proxy for data movement with only 4 links. In total, only 4 requests are needed for a batch. 
% Further, combined with request batching and aggregation, GraphScale can significantly reduce I/O workload.

%GL's design of feature fetching is a popular design choice. Most in-memory stores, such as Redis share the same approach, where the proxy node becomes one of the master nodes and the flow pattern are the same. One optimization to this design is that the topology sampling and feature fetching steps can be parallelized and the k-hop steps can also be pipelined, as shown by the authors in ByteGNN . 


%#Hops * #Sampler * #interactions


% \subsection{Training Graph Node Embeddings}
% The last step is to train mini-batch. The step requires a large amount of memory to store intermediate results of training, such as embedding or momentum. The cost of this step becomes nontrivial especially when the graph size is very large (e.g., embedding size of 128 with 1 billion node graph would require 500 GB of memory).

% {\bf Parameter Server}. 
% One approach to store distributed embedding is to use Parameter-server framework, such as Pytorch BigGraph. However this approach requires too much network bandwidth as each gradient update step, each trainer needs to issue a data transfer with PS. 




% {\bf Design goals of GraphScale}:
% GraphScale is designed to tackle the I/O bottleneck problem we discussed above. We want to achieve the following goals:

% \begin{itemize}[leftmargin=*]
% \setlength{\parskip}{0pt}
% \setlength{\itemsep}{0pt}
%     \item Efficient random access: The nature of the graph learning algorithm leads to lots of random data access (e.g., while feature-fetching during the sampling phase). 
%     In a distributed setup, cross-machine communication is also inevitable due to the multi-hop pattern of the graph, which is also random. 
%     \item High throughput: Mini-batch training  GNN models may require a larger number of features for each read/write operation (especially to support larger batch sizes). Hence, we want higher throughput.
%     \item High concurrency of data access: We would like to support multiple trainers reading and writing simultaneously. 
%     % \item Simple APIs to customize graph learning logic: This requires the support of update operations such as adding and multiplying to the stored data. Further, these APIs should be easily integrable into existing code. 
% \end{itemize}
% In our design of GraphScale, we address all the challenges above. 
% %Next, we present the system architecture of GraphScale in detail.



\subsection{GraphScale: System Architecture}

\begin{figure}[t]
\centering
%\includegraphics[scale=0.2]{result_figures/ROS_design.jpg}
\includegraphics[scale=0.23]{no_watermark/Flowchart-2.jpg}
\caption{GraphScale overview. MetaActor is responsible for data sharding, and ObjectActor stores the raw data (such as features and embeddings). Trainers store the entire graph topology and are responsible for computation over a subset of the graph (we show only one trainer for clarity). The thin lines represent the metadata flow, the dashed lines represent synchronization among MetaActors, and the solid lines represent raw data flow from ObjectActors to Trainers.}
\label{fig:ros_design_fig}
\end{figure}

Fig. \ref{fig:ros_design_fig} illustrates the system design of GraphScale. 
Throughout this paper, computation workers are referred to as Trainers, and workers who store the data are referred to as actors (similar to the terminology of Ray).
Actors are further subdivided into ObjectActors (workers that store large raw data) and MetaActors (workers that store small metadata). 
% Our insight to these challenges above is to design a generic and unified framework for all the data we may need during the GNN training, including features, embeddings and momentum. 
GraphScale is engineered to facilitate data partitioning, streamline data retrieval, and enable effective data updates. 
The foundational principles of GraphScale's design encompass three key aspects.
\begin{enumerate}[leftmargin=*]
\setlength{\parskip}{0pt}
\setlength{\itemsep}{0pt plus 0.2pt}
    \item {\bf Separate metadata and raw data}:
Metadata can be vertex indices, the ObjectActor ID, the shard index, or a reference to the raw data (typically small, in MegaBytes). The raw data (typically large, in GigaBytes or TeraBytes) can be graph data corresponding to nodes and edges, such as node features and embeddings.
In Fig. \ref{fig:ros_design_fig}, we show the two types of data flow corresponding to the two types of actors. 
The MetaActor stores the mapping between the vertex IDs to the IDs of ObjectActor. The ObjectActor stores the raw data in memory.
\item 
{\bf Minimize data movement}:
We believe that any raw data movement between MetaActor and ObjectActor is unnecessary. 
MetaActor is only responsible for retrieving the mappings. 
ObjectActor handles the data movement directly to trainers. 
If there is any update to the raw data, ObjectActor processes the update locally. 
\item 
% {\bf Reducing feature requests at trainers}:
% % Trainers save network bandwidth further by aggregating requests for features and processing them all at once at the end of the mini-batch. 
% Each trainer stores the entire graph topology, and after processing a subgraph during mini-batch training, it aggregates vertices to deduplicate vertex IDs before sending (only one) request for features to the MetaActors.
% ObjectActor constructs a single data block per request and sends it to the trainer. Aggregating requests and deduplicating vertices from multiple requests significantly reduces network bandwidth utilization.
{\bf Minimizing network load in training}: To use network bandwidth more efficiently, trainers combine multiple feature requests into a single batch at the end of each mini-batch training session. By keeping the entire graph topology, trainers can merge the same vertex IDs from subgraphs before making a single feature request to the MetaActors. The ObjectActor then responds with just one data block per request. This method of consolidating requests and removing duplicate vertices greatly reduces the network bandwidth needed.
\end{enumerate}




Next, we describe how the GraphScale system architecture supports basic operations such as reading and writing.
During the {\bf read operation}, 
The trainer first buffers all requests per training batch and deduplicates the vertices before sending the request to MetaActor. Each trainer is designated to a MetaActor for load balancing. It will route all requested vertex IDs to the corresponding ObjectActor. Once the requests are received, the ObjectActor constructs a data block and returns a reference to the trainer. The trainer then starts the data transfer from all ObjectActors asynchronously.

%reduce the number of internal requests and avoid unnecessary data movement.
During the {\bf update operation}, 
the trainer first retrieves the mapping information from MetaActor. The new values will be partitioned based on the mapping and then written to ObjectActor. Here, each ObjectActor maintains a sorted list of keys to speed up the lookup process. 
Since we have multiple MetaActors, the new mapping will be automatically synchronized among them. This process happens asynchronously while the data is being written to the ObjectActors; thus, it incurs almost no overhead.

GraphScale also supports some other simple computations, such as add and multiply. These operations are similar to the update operation we described above. 
The only difference is that once the ObjectActor receives the new data, the simple computations happen locally and then update the values. The next section describes these operations in detail, where we utilize GraphScale for node embedding training.

==> ros_overview_simple.tex <==


% \section{GraphScale: An Overview}
% \section{Preliminaries}
\section{GraphScale for Training GNNs}
\label{sec:ros_design}
In this section, we first review the basics of GNN training. 
% Then, we motivate the design goals of GraphScale, followed by describing its system architecture.
Then, we describe how GraphScale assists in fast-distributed GNN training.
% We review feature fetching step and training step with Graph learn, PyTorch BigGraph and PyTorch DDP. 


{\bf I/O bottleneck during GNN Training}. Mini-batch processing in Graph Neural Network (GNN) training can be divided into three main steps: (1) Sampling a subgraph from the original graph. The result is the vertex and edge IDs of the sampled nodes and edges, respectively. (2) Feature fetching corresponding to vertex/edge IDs of the sampled nodes/edges in the sub-graph, and (3) Training the GNN for that mini-batch using the sub-graph topology, and the features and labels for corresponding nodes and edges.

% {\bf I/O bottleneck from feature fetching}. Existing GNN training frameworks suffer from data I/O bottlenecks. 
% % Two representative distributed GNN training frameworks are 
% The two notable distributed GNN training systems, Graphlearn (GL)\footnote{ByteGNN \cite{bytegnn} is a further optimized version of Graphlearn, where sampling and feature fetching are phases of GNN training are parallelized, and the k-hop neighbor fetching is pipelined.} \cite{aligraph} and DistDGL \cite{dist_dgl}, both rely on a similar underlying architecture for feature fetching.
% % (as illustrated in Fig. \ref{fig:gl_feature_fetch}).
% % DistDGL is based on a generic K/V store to fetch features. 
% For each sampling request per mini-batch, the respective graph backend issues a request to fetch features for the sampled vertices.
% % We observe a common limitation in both frameworks. 
% This design is inefficient due to two reasons. First, it processes a large number of requests to fetch features for a single batch, which might cause significant network congestion.
% Second, the requests of neighboring hops are highly likely to have duplicate vertices due to the power-law attribute of the graph, but features for each vertex may be included in multiple requests leading to a heavy network workload. 
% %We give a specific example of this at the end of next section.

Current distributed training frameworks for GNNs suffer from data communication bottlenecks. Both Graphlearn (GL) \footnote{ByteGNN \cite{bytegnn} is a further optimized version of Graphlearn, where sampling and feature fetching are phases of GNN training are parallelized, and the k-hop neighbor fetching is pipelined.} \cite{aligraph} and DistDGL \cite{dist_dgl}, which are prominent distributed GNN training systems, exhibit a shared architectural approach in feature fetching. The process involves issuing requests from the graph backend to retrieve features for sampled vertices in each mini-batch. This methodology is inefficient for two primary reasons. Firstly, it generates a high volume of feature-fetching requests for each batch, potentially causing high network traffic. Secondly, due to the graph's power-law distribution, there is a high probability of duplicated vertices in neighboring hops. However, the system often processes features for these repeated vertices multiple times, resulting in increased network load. This is illustrated in Fig. \ref{fig:gnn_comm_bottleneck}. 
\yy{This part is good, and can be used as a subsection about background of GNN training in the Preliminaries section. 
I would arrange the Preliminaries section like this: (a). move the notation part up and use it as the first subsection. Only label notations need to be mentioned here (e.g., G, V, E, N, d M, n). If you also use any label notions for GNNs, also put it here. Other parts in the notation section relate more to the background of embedding training, which should be mentioned later. (b). The second subsection should be traditional embedding training, where you can say how embeddings are trained in more detail. This subsection should contain some contents you mention in section 3, including the introduction of DDP, but you need to leave out the modifications specific to GraphScale. (c). The third subsection should be traditional GNN training, and I think you can directly put the above subsection (I/O bottleneck during GNN training) here. All the contents about GraphScale should go to section 3. My thoughts on the organization of section 3: (a) An overview of the GraphScale framework you proposed, mentioning several key designs. This paragraph should be very high level. What are different building blocks (e.g. briefly introducing trainers and workers and their functionality)? what does separation of storage and computation mean? What does asynchronization mean and how do you achieve it in practice? This part should be very concise and just touch upon the whole pipeline and mention some key designs.(b) Subsection 1, storage and computation separation. First go with the intuition, something you mention in ``GraphScale system design" and ``Reducing feature requests by trainers" should fit here. Just give the rationale why GraphScale can reduce communication costs. Then elaborate it a bit by providing more details. Here you can split into two parts: how do you achieve the storage and computation separation in embeddging training and how does it save the time; how do you achieve it in GNN training (most of the contents in ``Reducing feature requests by trainers" should fit here) and how does that save time? In this subsection, you can also refer to the premilary section and point out the key difference, e.g., differences from DDP.
Subsection 2, Gradient updates. Put the last paragraph in page 4 and synchronization here. }

{\bf GraphScale system design}. In GraphScale, our reimagined system architecture for GNN training capitalizes on the separation of storage and computation. 
Throughout this paper, computation workers are referred to as trainers, and workers who store the data are referred to as actors (similar to the terminology of Ray).
Separating storage actors and trainers drastically cuts down communication overhead, as it necessitates only a single feature request for the sub-graph from each trainer. This efficiency is largely enabled by Ray's capacity to facilitate an easy abstraction of storage and computation in serverless systems.
% GraphScale is engineered to facilitate data partitioning and streamline data retrieval. 
GraphScale storage actors also enable effective data updates by allowing operations like read, update, addition, and multiplication.

{\bf Reducing feature requests by trainers}. To use network bandwidth efficiently during GNN training with GraphScale, trainers combine multiple feature requests into a single batch at the end of each mini-batch training session. By keeping the entire graph topology, trainers can merge the same vertex IDs from subgraphs before making (a single) feature request to the actors. The actors then respond with one data block per request. This method of consolidating requests and removing duplicate vertices greatly reduces the network bandwidth needed. This also reduces the dependence on the partitioning scheme, since regardless of the partition, only one communication request is needed per trainer. However, the size of the data to be communicated still depends on the partitioning scheme, but its effect on the overall training time is negligible.

% The foundational principles of GraphScale's design encompass three key aspects.
% \begin{enumerate}[leftmargin=*]
% \setlength{\parskip}{0pt}
% \setlength{\itemsep}{0pt plus 0.2pt}
%     \item {\bf Separate metadata and raw data}:
% Metadata can be vertex indices, the ObjectActor ID, the shard index, or a reference to the raw data (typically small, in MegaBytes). The raw data (typically large, in GigaBytes or TeraBytes) can be graph data corresponding to nodes and edges, such as node features and embeddings.
% In Fig. \ref{fig:ros_design_fig}, we show the two types of data flow corresponding to the two types of actors. 
% The MetaActor stores the mapping between the vertex IDs to the IDs of ObjectActor. The ObjectActor stores the raw data in memory.
% \item 
% {\bf Minimize data movement}:
% We believe that any raw data movement between MetaActor and ObjectActor is unnecessary. 
% MetaActor is only responsible for retrieving the mappings. 
% ObjectActor handles the data movement directly to trainers. 
% If there is any update to the raw data, ObjectActor processes the update locally. 
% \item 
% % {\bf Reducing feature requests at trainers}:
% % % Trainers save network bandwidth further by aggregating requests for features and processing them all at once at the end of the mini-batch. 
% % Each trainer stores the entire graph topology, and after processing a subgraph during mini-batch training, it aggregates vertices to deduplicate vertex IDs before sending (only one) request for features to the MetaActors.
% % ObjectActor constructs a single data block per request and sends it to the trainer. Aggregating requests and deduplicating vertices from multiple requests significantly reduces network bandwidth utilization.
% {\bf Minimizing network load in training}: To use network bandwidth more efficiently, trainers combine multiple feature requests into a single batch at the end of each mini-batch training session. By keeping the entire graph topology, trainers can merge the same vertex IDs from subgraphs before making a single feature request to the MetaActors. The ObjectActor then responds with just one data block per request. This method of consolidating requests and removing duplicate vertices greatly reduces the network bandwidth needed.
% \end{enumerate}




% Next, we describe how the GraphScale system architecture supports basic operations such as reading and writing. During the {\bf read operation}, The trainer first buffers all requests per training batch and deduplicates the vertices before sending the request to MetaActor. Each trainer is designated to a MetaActor for load balancing. It will route all requested vertex IDs to the corresponding ObjectActor. Once the requests are received, the ObjectActor constructs a data block and returns a reference to the trainer. The trainer then starts the data transfer from all ObjectActors asynchronously.

% During the {\bf update operation}, the trainer first retrieves the mapping information from MetaActor. The new values will be partitioned based on the mapping and then written to ObjectActor. Here, each ObjectActor maintains a sorted list of keys to speed up the lookup process. 
% Since we have multiple MetaActors, the new mapping will be automatically synchronized among them. This process happens asynchronously while the data is being written to the ObjectActors; thus, it incurs almost no overhead.

% GraphScale also supports some other simple computations, such as add and multiply. These operations are similar to the update operation we described above. The only difference is that once the ObjectActor receives the new data, the simple computations happen locally and then update the values. The next section describes these operations in detail, where we utilize GraphScale for node embedding training.
